Assessment of Multimodal Large Language Models in Alignment with Human Values

Large Language Models (LLMs) aim to serve as versatile assistants aligned with human values, as defined by the principles of being helpful, honest, and harmless (hhh). However, in terms of Multimodal Large Language Models (MLLMs), despite their commendable performance in perception and reasoning tasks, their alignment with human values remains largely unexplored, given the complexity of defining hhh dimensions in the visual world and the difficulty in collecting relevant data that accurately mirrors real-world situations. To address this gap, we introduce Ch3Ef, a Compreh3ensive Evaluation dataset and strategy for assessing alignment with human expectations. Ch3Ef dataset contains 1002 human-annotated data samples, covering 12 domains and 46 tasks based on the hhh principle. We also present a unified evaluation strategy supporting assessment across various scenarios and different perspectives. Based on the evaluation results, we summarize over 10 key findings that deepen the understanding of MLLM capabilities, limitations, and the dynamic relationships between evaluation levels, guiding future advancements in the field.

==> sections/authors.tex <==
% % TODO FINAL: Replace with your author list. 
% % Include the authors' OCRID for the camera-ready version, if at all possible.
% \author{First Author\inst{1}\orcidlink{0000-1111-2222-3333} \and
% Second Author\inst{2,3}\orcidlink{1111-2222-3333-4444} \and
% Third Author\inst{3}\orcidlink{2222--3333-4444-5555}}

% % TODO FINAL: Replace with an abbreviated list of authors.
% \authorrunning{F.~Author et al.}
% % First names are abbreviated in the running head.
% % If there are more than two authors, 'et al.' is used.

% % TODO FINAL: Replace with your institution list.
% \institute{Princeton University, Princeton NJ 08544, USA \and
% Springer Heidelberg, Tiergartenstr.~17, 69121 Heidelberg, Germany
% \email{lncs@springer.com}\\
% \url{http://www.springer.com/gp/computer-science/lncs} \and
% ABC Institute, Rupert-Karls-University Heidelberg, Heidelberg, Germany\\
% \email{\{abc,lncs\}@uni-heidelberg.de}}


\makeatletter
\renewcommand*{\@fnsymbol}[1]{\ifcase#1\or*\or\dag\or\ddag\fi}
\makeatother

\makeatletter
\newcommand{\printfnsymbol}[1]{%
  \textsuperscript{\@fnsymbol{#1}}%
}
\makeatother

\author{
    Zeren Chen\inst{1,3}\thanks{Equal contribution.} \and
    Zhelun Shi\inst{1,3}\printfnsymbol{1} \and
    Xiaoya Lu\inst{1,5}\printfnsymbol{1} \and
    Lehan He\inst{1,6}\printfnsymbol{1} \and
    Sucheng Qian\inst{1,2} \and
    Hao Shu Fang\inst{2} \and
    Zhenfei Yin\inst{1,4}\thanks{Project leader.} \and
    Wanli Ouyang\inst{1,4} \and \\
    Jing Shao\inst{1}\thanks{Corresponding author.} \and
    Yu Qiao\inst{1} \and
    Cewu Lu\inst{2} \and
    Lu Sheng\inst{3}\printfnsymbol{3}
}


\institute{
    Shanghai AI Laboratory \and
    Shanghai Jiao Tong University \and
    Beihang University \and
    University of Sydney \and 
    University of Electronic Science and Technology of China \and
    Nanjing University of Posts and Telecommunications
}
